Secure Group Testing

The principal goal of Group Testing (GT) is to identify a small subset of "defective" items from a large population, by grouping items into as few test pools as possible. The test outcome of a pool is positive if it contains at least one defective item, and is negative otherwise. GT algorithms are utilized in numerous applications, and in many of them maintaining the privacy of the tested items, namely, keeping secret whether they are defective or not, is critical. In this paper, we consider a scenario where there is an eavesdropper (Eve) who is able to observe a subset of the GT outcomes (pools). We propose a new non-adaptive Secure Group Testing (SGT) scheme based on information-theoretic principles. The new proposed test design keeps the eavesdropper ignorant regarding the items' status. Specifically, when the fraction of tests observed by Eve is $0 \leq \delta <1$, we prove that with the naive Maximum Likelihood (ML) decoding algorithm the number of tests required for both correct reconstruction at the legitimate user (with high probability) and negligible information leakage to Eve is $\frac{1}{1-\delta}$ times the number of tests required with no secrecy constraint for the fixed $K$ regime. By a matching converse, we completely characterize the Secure GT capacity. Moreover, we consider the Definitely Non-Defective (DND) computationally efficient decoding algorithm, proposed in the literature for non-secure GT. We prove that with the new secure test design, for $\delta < 1/2$, the number of tests required, without any constraint on $K$, is at most $\frac{1}{1/2-\delta}$ times the number of tests required with no secrecy constraint.

==> WeakSecure.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\tifs{Information Leakage at the Eavesdropper\\ (Weak Secrecy)}}\label{LowerBoundLeakage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We now prove the \tifs{weak} security constraint is met. Hence, we wish to show that $I(W;Z^{T})/T\rightarrow 0$, as $T\rightarrow \infty$.
Denote by $\mathcal{C}_T$ the random codebook and by $X_{\mathcal{S}}^T$ the set of codewords corresponding to the true, defective items set $\mathcal{S}$, given $W$ and the corresponding function $(W;R_K) \rightarrow X^{T}_{\mathcal{S}}$. We have,
\begin{eqnarray}
&& \hspace{-0.8cm}\textstyle\textstyle \frac{1}{T}I(W;Z^T|\mathcal{C}_{T}) = \frac{1}{T}\left(I(W,R_K;Z^T|\mathcal{C}_{T})-I(R_K;Z^T|W,\mathcal{C}_{T})\right)\nonumber\\
&\hspace{-0.6cm}  \stackrel{(a)}{\leq} &\hspace{-0.5cm}\textstyle \frac{1}{T}\left(I(X_{\mathcal{S}}^T;Z^T|\mathcal{C}_{T})-I(R_K;Z^T|W,\mathcal{C}_{T})\right)\nonumber\\
&\hspace{-0.6cm} = &\hspace{-0.5cm}\textstyle \frac{1}{T}(I(X_{\mathcal{S}}^T;Z^T|\mathcal{C}_{T})-H(R_K|W,\mathcal{C}_{T})+H(R_K|Z^T,W,\mathcal{C}_{T}))\nonumber\\
&\hspace{-0.6cm} \stackrel{(b)}{=} & \hspace{-0.5cm}\textstyle \frac{1}{T}\left(I(X_{\mathcal{S}}^T;Z^T|\mathcal{C}_{T})-H(R_K)+H(R_K|Z^T,W,\mathcal{C}_{T})\right)\nonumber\\
&\hspace{-0.6cm} \stackrel{(c)}{\leq}&\hspace{-0.5cm} I(X_{\mathcal{S}};Z|\mathcal{C}_{T}) - \frac{1}{T}K\log M + \frac{1}{T}H(R_K|Z^T,W,\mathcal{C}_{T})\label{eq:leak_apply}\hspace{-0.2cm}\\
&\hspace{-0.6cm} \stackrel{(d)}{\leq}&\hspace{-0.5cm} \delta - \frac{1}{T}K\left(T \frac{\delta-\epsilon^{\prime}}{K}\right) + \frac{1}{T}H(R_K|Z^T,W,\mathcal{C}_{T})\stackrel{(e)}{\leq} \epsilon_T + \epsilon^{\prime},\nonumber
%&\hspace{-0.7cm} \stackrel{(e)}{\leq}&\hspace{-0.5cm} \epsilon_T,\nonumber
\end{eqnarray}
where $\epsilon_T \to 0$ as $T \to \infty$\. (a) is since $(W;R_K) \rightarrow X^{T}_{\mathcal{S}} \rightarrow Z^T$; note that given $\mathcal{C}_{T}$ there is a function correspondence between $(W,R_K)$ and $X_{\mathcal{S}}^T$, the mapping of the defective set and the internal randomness to the codewords used. It is important to note that since the codebook is generated randomly, the mapping is not exactly $1:1$ and there is a possibility for a repetition of codewords. However, averaged over all the possible sets of defective items $W$, the error probability from such a repetition is negligible, and this is a direct consequence using standard analysis of random coding given in \cite[Section 3.4]{C13}; (b) is since $R_K$ is independent of $W$ and $\mathcal{C}_T$; (c) is since the channel is memoryless, hence $I(X_{\mathcal{S}}^T;Z^T|\mathcal{C}_{T}) \leq T I(X_{\mathcal{S}};Z|\mathcal{C}_{T})$. This is a standard application of, e.g., \cite[Lemma 7.9.2]{cover2012elements}; (d) is since by choosing \tifs{$M =2^{\left(\frac{\delta-\epsilon^{\prime}}{K}\right)T}$ and} an i.i.d.\ distribution for the random codebook, when $H(R_K)=\log(M^K)$ and $R_K$ is chosen random and independent at the mixer, one easily observes that $I(X_{\mathcal{S}};Z| \mathcal{C}_T) \leq \delta$. For (e), bounding $H(R_K|Z^T,W,\mathcal{C}_T)$, we wish to show that \emph{given the set of defective items, the codebook, and the information Eve has}, she can infer the internal randomess used with a low error probability. This is, in a sense, similar to wiretap coding or secure network coding, where the message itself is concealed from Eve, using the internal randomness, \emph{yet given the message, Eve can easily guess the internal randomness used}. Now, for the specific case herein: The codebook is known to all. Any party knowing $W$, knows which were the defective items (from which bins the codewords were taken). We claim that this situation is \emph{analogous to a noiseless Boolean Multiple Access Channel, followed by an erasure channel}. To see this, note that there are $K$ defectives. Each of these (a ``user", in the analogy) puts a codeword on the channel. The codewords are summed. Then, Eve sees the sum through an erasure channel, since she sees only a fraction $\delta$. We wish to show that Eve can decode, i.e., know which codeword each defective item has put on the channel, hence get the internal randomness. The channel capacity is $\delta$. There are $K$ users. Thus, a rate of $\delta/K$ is attainable for each user. Since the block size is $T$, each user can have (a bit less than) $2^{T(\frac{\delta}{K})}$ codewords and Eve can still infer which codeword each user transmitted. $\epsilon_T$ is Eve's (the decoder) error probability, and by Fano's inequality $H(R_K|Z^T,W,\mathcal{C}_T) \leq T \epsilon_T$. Finally, all that is left to explain is that the codewords used for SGT are also good to attain the capacity for this \tifs{Multiple Access Channel (MAC)}. The distribution used herein is i.i.d. with probabilities  $(\frac{\ln(2)}{K},1-\frac{\ln(2)}{K})$\tifs{\footref{note10}}. The MAC requires i.i.d. with probabilities $(1-2^{\frac{1}{K}}, 2^{\frac{1}{K}})$, but since the mutual information is continuous in the input distribution, this holds.

\begin{remark}
Under non-secure GT, it is clear that simply adding tests to a given GT code (increasing $T$) can only improve the performance of the code (in terms of reliability). A legitimate decoder can always disregard the added tests. For SGT, however, the situation is different. Simply adding tests to a given code, \emph{while fixing the bin sizes}, might make the vector of results vulnerable to eavesdropping. In order to increase reliability, one should, of course, increase $T$, but also increase the bin sizes proportionally, so the secrecy result above will still hold. This will be true for the efficient algorithm suggested in \Cref{efficient_algorithms} as well.
\end{remark}

\begin{remark}
Note that since
\begin{eqnarray*}
  \frac{1}{T}H(R_K|Z^T,W,\mathcal{C}_{T}) \hspace{-0.2cm} &=\hspace{-0.2cm}& \frac{1}{T}H(R_K)-\frac{1}{T}I(R_K;Z^T,W,\mathcal{C}_{T}) \\
   \hspace{-0.2cm}&=\hspace{-0.2cm}& \frac{1}{T}\tifs{K}\log M - \frac{1}{T}I(R_K;Z^T,W,\mathcal{C}_{T}),
\end{eqnarray*}
any finite-length approximation for $I(R_K;Z^T,W,\mathcal{C}_{T})$ will give a finite length approximation for the leakage at the eavesdropper.
For example, one can use the results in \cite{polyanskiy2010channel}, to show that the leakage can be approximated as $\frac{1}{\sqrt{T}}+\epsilon^{\prime}$.
\end{remark}
